Stochastic Shadowing and Stochastic Stability

The notion of stochastic shadowing property is introduced. Relations to stochastic stability and standard shadowing are studied. Using tent map as an example it is proved that, in contrast to what happens for standard shadowing, there are significantly non-uniformly hyperbolic systems that satisfy stochastic shadowing property.

==> preamble.tex <==
\newcommand{\Rb}{\mathbb R}
\newcommand{\Nb}{\mathbb N}
\newcommand{\Zb}{\mathbb Z}
\newcommand{\Lc}{\mathcal L}
\newcommand{\eps}{\varepsilon}
\newcommand{\dx}{\textbf{dx}}
\newcommand{\lb}{\left(}
\newcommand{\rb}{\right)}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\diff}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\diffd}[2]{\frac{\partial^2}{\partial #1 \partial #2}}
\newcommand{\sumd}[2]{\sum_{u = #1}^{#2}}
\newcommand{\ceilr}{\lceil r \rceil}
\newcommand{\floor}[1]{\lfloor #1 \rfloor}
\newcommand{\enbrace}[1]{\lb #1 \rb}
\newcommand{\inv}[1]{#1^{-1}}
\newcommand{\setdef}[2]{\left\{ #1\ \left\lvert\ #2 \right.\right\}}
\newcommand{\seqz}[2]{\left\{ {#1}_{#2} \right\}_{#2\in\Zb}}
\newcommand{\seq}[1]{ \left\{ #1 \right\} }

\newcommand{\half}[1]{\frac{#1}{2}}

\newcommand{\vmod}[1]{\left| #1 \right|}
\newcommand{\linhull}[1]{\left< #1 \right>}

\newcommand{\Nc}{\mathcal{N}}
\newcommand{\normB}[1]{\left\| #1 \right\|_\infty}

\newcommand{\normop}[1]{\left\| #1 \right\|}
\newcommand{\normban}[1]{\left\| #1 \right\|}

%\newcommand{\emk}{\exp^{-1}_{p_{k+1}}}
%\newcommand{\ekk}{\exp_{p_{k+1}}}
%\newcommand{\ekki}{\exp^{-1}_{p_{k+1}}}
\newcommand{\Nint}{[-N,N-1]} %for eqs
\newcommand{\Nintw}{[-N+1,N]} %for inhoms
\newcommand{\Nints}{[-N,N]} %for solutions
\newcommand{\Ninta}{[0,2N]} %for solutions
\newcommand{\Nintanz}{[1,2N]} %for solutions

\newcommand{\enkav}[1]{``#1''}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newlength{\negskiplength}
\setlength{\negskiplength}{0.07em}
\newcommand{\negskip}{\hskip-\negskiplength}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%  on manifold

\newcommand{\expi}[1]{\exp_{#1}^{-1} }
\newcommand{\ekM}[2]{ \exp_{p_{#1} } \enbrace{#2} }
\newcommand{\ekiM}[2]{\exp_{p_{#1} }^{-1} \enbrace{#2} }
\newcommand{\ebaseptM}[1]{\ekM{\baseptind}{#1}}
\newcommand{\tvM}{\ebaseptM{v}}

%\renewcommand{\eshM}[2]{\ek{#1}(#2)}
\newcommand{\emultM}{2}

\newcommand{\mfdM}{ M } %M
\newcommand{\tgtM}[1]{ T_{p_{#1}} \mfdM } %{ \Rb^n } % T_{p_{#1}} M
\newcommand{\ekPM}[1]{ \exp_{p_{#1}} }   % ek proto



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%  for R^n

%\newcommand{\esh}[2]{\ek{#1}(#2)}
\newcommand{\emult}{}

\newcommand{\tgt}[1]{ \Rb^n } % T_{p_{#1}} M
\newcommand{\mfd}{ \Rb^n } %M
\newcommand{\ekP}[1]{ p_{#1}}   % ek proto
\newcommand{\ek}[2]{ \ekP{#1} + {#2} }
\newcommand{\eki}[2]{ -\ekP{#1} + {#2} }

%\newcommand{\ekP}[1]{ p_{#1}}   % ek proto

%\renewcommand{\ek}[2]{ p_{#1} + {#2} }
%\renewcommand{\eki}[2]{ -p_{#1} + {#2} }
%
%\renewcommand{\esh}[2]{p_{#1}+ #2}
%\renewcommand{\emult}{}

%\renewcommand{\tgt}[1]{ \Rb^n } % T_{p_{#1}} M
%\renewcommand{\mfd}{ \Rb^n } %M


\newcommand{\dmettime}{1}
\newcommand{\vfield}{X}
\newcommand{\dmet}{\Psi}
\newcommand{\dmetsupp}{\Theta}
\newcommand{\dmetk}[1]{\dmet } %\dmet^{(#1)}
\newcommand{\flow}{\Phi}
\newcommand{\dmetclassletter}{$\mathcal{T}$}
\newcommand{\dmetclass}[1]{\mathcal{T}_{#1}}
\newcommand{\dmetMap}{\tilde{\dmet}}
\newcommand{\linsol}[2]{\Delta^{(#1)}_{#2}}
\newcommand{\tzero}{1}
\newcommand{\Rep}{\mathrm{Rep}}
\newcommand{\Repe}[1]{\Rep\enbrace{#1} }
\newcommand{\smtclass}{1}
\newcommand{\eqconst}{\Lone}

\newcommand{\dadd}{^{(d)}}

\newcommand{\baseptind}{-N}
\newcommand{\basept}{p_{\baseptind}}
\newcommand{\baseptk}[1]{p_{#1}}
\newcommand{\ekbP}[1]{p_{#1}}
\newcommand{\ebasept}[1]{\ek{\baseptind}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dm}{ \dmet_{ \varkappa } }
\newcommand{\dms}{ \dmetsupp_{ \varkappa } }

\newcommand{\dmz}{ \dmet_{0} }
\newcommand{\dmsz}{ \dmetsupp_{ 0 } }
\newcommand{\dmo}{ \dmet_{1} }
\newcommand{\dmso}{ \dmetsupp_{1} }
\newcommand{\dmod}{ \dmet_{1}\dadd }
\newcommand{\dmsod}{ \dmetsupp_{1}\dadd }

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%  for R^n


%\newcommand{\ekbpt}[2]{\ek{\baseptind+ {#1}  }{#2} }
%\newcommand{\ekibpt}[2]{\eki{\baseptind+ {#1} }{#2} }


\newcommand{\npk}[1]{ \tilde{p}_{ #1} }
\newcommand{\nAk}[1]{ \tilde{A}_{ #1} }
\newcommand{\nnpk}[1]{ \hat{p}_{  #1} }
\newcommand{\npkd}[1]{ \tilde{p}_{ #1}\dadd }
\newcommand{\nAkd}[1]{ \tilde{A}_{ #1}\dadd }
\newcommand{\nnpkd}[1]{ \hat{p}_{  #1}\dadd }

\newcommand{\om}[1]{\Omega_{\varkappa,#1} }
\newcommand{\omod}[1]{\Omega_{1,#1}\dadd }


\newcommand{\oned}{\frac{1}{d}}
\newcommand{\tdiff}{\sigma\dadd} 
\newcommand{\tdiffoned}{s\dadd }
\newcommand{\tdiffonedfin}{s^* }
\newcommand{\reparam}{\beta\dadd}
\newcommand{\reparamz}{\alpha}
\newcommand{\repz}{a}

\newcommand{\shdt}{y\dadd}  % shadowing discrete trajectory
\newcommand{\shdtz}{x}  % shadowing discrete trajectory
\newcommand{\shadptz}{p^*}
\newcommand{\shadptnodadd}{\hat{p}}
\newcommand{\shadpt}{\hat{p}\dadd}
\newcommand{\vd}{v\dadd}
\newcommand{\vdz}{q}
\newcommand{\tv}{\ebasept{v}}
\newcommand{\tvd}{\ebasept{\vd}}
\newcommand{\tvdz}{\ebasept{\vdz}}
\newcommand{\vres}{w\dadd}
\newcommand{\vpreres}{W\dadd}
\newcommand{\vfin}{w^*}

\newcommand{\timedevkz}{\reparamz{k}-k}
\newcommand{\timedevko}{\reparam{k}-k}

\newcommand{\ldz}{\lim_{d\to 0}}

%\newcommand{\osmOmega}{g_2\dadd }
\newcommand{\osmX}{ g_1 }
\newcommand{\osmIC}{ g_2}
\newcommand{\osmTaylorRem}{ g_2 }
\newcommand{\taufun}{ \tilde{g} }

\newcommand{\distletter}{\delta}
\newcommand{\constdmet}{C_{\varkappa}(d)}
\newcommand{\constdmetz}{C_{0}(d)}
\newcommand{\constdmeto}{C_{1}(d)}

%%%%%% global flow constants
\newcommand{\maxderiv}{Q_1}
\newcommand{\maxvfield}{Q_2}
\newcommand{\maxshearflow}{Q_3}
\newcommand{\maxdiv}{Q_4}

\newcommand{\constpknpk}{K_5}
%\newcommand{\maxdivmet}{Q_5}
%\newcommand{\maxshearmet}{Q_5}

\newcommand{\kaocond}{if $\varkappa = 1$ then}
\newcommand{\kazcond}{if $\varkappa = 0$ then}
 

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\rayp}{{\Zb^+}}
\newcommand{\rayn}{{\Zb^-}}

\newcommand{\RP}{\mathcal{RP}}
\newcommand{\CR}{\mathcal{CR}}


\newcommand{\ruemd}{--}% "---} %russian em-dash

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\diam}{diam}
\DeclareMathOperator{\Diff}{Diff}
\DeclareMathOperator{\LISP}{LISP}
\DeclareMathOperator{\Id}{Id}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\numberwithin{equation}{section}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\theoremstyle{plain}
 \newtheorem{theorem}{Theorem}
 \newtheorem*{theoremnon}{Theorem}
 \newtheorem{statement}{Statement}[section]
 \newtheorem{lemmaa}[statement]{Lemma}
 \newtheorem{corollary}[statement]{Corollary}
\theoremstyle{definition} \newtheorem{deff}{Definition}
 \newtheorem*{deffnon}{Definition}
\theoremstyle{remark} \newtheorem{rem}[statement]{Remark}

